Search for the Decays B0->e+e-gamma and B0->mu+mu-gamma

We present results of a search for the decays $B^0 \to \ell^+\ell^-\gamma$ ($\ell=e$, $\mu$). The search is performed using $320\times 10^{6}$ $B\bar{B}$ pairs collected at the $\Upsilon(4S)$ resonance with the BABAR detector at the PEP-II $B$ Factory at SLAC. We find no significant signal and set the following branching fraction upper limits at the 90% confidence level: $\mathcal{B}(B^0\to e^+e^-\gamma)<1.2\times 10^{-7}$ and $\mathcal{B}(B^0\to \mu^+\mu^-\gamma)<1.5\times 10^{-7}$.

==> abstract.tex <==
We present results of a search for the decays $B^0 \rightarrow \ell^+\ell^-\gamma$ ($\ell=e$, $\mu$).  The search is performed using $320\times 10^{6}$ $B\bar{B}$ pairs collected at the $\Upsilon(4S)$ resonance with the BABAR detector at the PEP-II $B$ Factory at SLAC. We find no
significant signal and set the following branching fraction upper limits at the
90\% confidence level: $\mathcal{B}(B^0\rightarrow
e^+e^-\gamma)<1.2\times 10^{-7}$ and $\mathcal{B}(B^0\rightarrow
\mu^+\mu^-\gamma)<1.5\times 10^{-7}$.

